Forward BFKL evolution at fixed coupling as a random walk, and the loss of its probability law at fixed next-to-leading order

The BFKL equation describes how the density of gluons in a hadron grows with the collision energy. This evolution is often treated as a random walk in the logarithm of the gluon transverse momentum, but it has not been established that one set of positive step probabilities describes this walk in the size and the direction of the momentum, or that such probabilities exist beyond leading order. We show that one positive step density describes the evolution in the size and the direction of the momentum with no approximation at leading order, fixed coupling and zero momentum transfer, once the gluon density is rescaled by the size of its transverse momentum and its growth is divided out. The displacements of the resulting walk over separate, equal intervals of rapidity, the logarithm of the energy in units of a reference energy, are then independent and identically distributed, which makes the walk a Levy process. We also show that this description fails when the series in the coupling is cut at next-to-leading order, with the reference energy and the scale of the coupling both set by the product of the transverse momenta before and after an emission. The evolution averaged over directions then has no probability law at any fixed positive coupling and rapidity, because a negative correction growing as the squared logarithm of the momentum ratio outweighs the leading term when one momentum is much larger than the other. A positive step density for the averaged walk agrees with this truncated evolution to next-to-leading order and defines a random walk for every value of the strong coupling below one, so the failure comes from the truncation. The main message is that agreement with perturbation theory does not guarantee positive step probabilities, so an evolution equation summed to all orders and meant to describe a random walk must be tested for them.

==> macros-v2.tex <==
% ------------------------------------------------------------------
% macros-v2.tex : printed numbers, computed at N_c = 3, n_f = 4.
% A stored artifact: the program that wrote it is not in this archive.
% Do not hand-edit the numbers.  The comments are maintained by hand.
% ------------------------------------------------------------------

% --- Laurent coefficients of chi_1 (exact rationals where exact) ---
\newcommand{\dthirteen}{-\tfrac12}
\newcommand{\dtwelve}{-1.28858025}
\newcommand{\deleven}{-0.423868313}
\newcommand{\ethirteen}{-\tfrac12}
\newcommand{\etwelve}{-0.0206790123}
\newcommand{\eleven}{2.46387252}
\newcommand{\fthirteen}{-\tfrac12}
\newcommand{\ftwelve}{-0.540961199}
\newcommand{\feleven}{2.74592761}
\newcommand{\bbarval}{0.69444444}
\newcommand{\Kval}{2.6730948}

% --- converged full-density sign-change roots, not printed in this paper ---
% bracketed + Newton to a fixed point; three independent inversions
% (exact residue/layer sum, rotated contour, cosine transform with the
% analytic ln^2 nu tail) agree to better than 1\times10^{-12}.  Uncertainty 1\times10^{-9}.
\newcommand{\rootA}{6.642667798}
\newcommand{\rootAfull}{6.642667797519045}
\newcommand{\rootB}{4.164653922}
\newcommand{\rootBfull}{4.164653922219484}
\newcommand{\rootC}{2.596542267}
\newcommand{\rootCfull}{2.596542267083477}
\newcommand{\rootD}{2.019482361}
\newcommand{\rootDfull}{2.019482360877770}
\newcommand{\rootunc}{1\times10^{-9}}

% --- root residuals, normalized residuals and differences, entries A to D ---
\newcommand{\vonerootresA}{-1.11\times10^{-10}}
\newcommand{\vonerootresnormA}{-1.11\times10^{-10}}
\newcommand{\vonerootdiffA}{4.81\times10^{-10}}
\newcommand{\vonerootresB}{7.63\times10^{-11}}
\newcommand{\vonerootresnormB}{7.75\times10^{-11}}
\newcommand{\vonerootdiffB}{-2.19\times10^{-10}}
\newcommand{\vonerootresC}{-1.4\times10^{-7}}
\newcommand{\vonerootresnormC}{-1.51\times10^{-7}}
\newcommand{\vonerootdiffC}{2.37\times10^{-7}}
\newcommand{\vonerootresD}{-1.44\times10^{-5}}
\newcommand{\vonerootresnormD}{-1.66\times10^{-5}}
\newcommand{\vonerootdiffD}{1.69\times10^{-5}}

% --- the C bound at x_0 = 2.35, rounded upward to five decimals,
%     not printed in this paper ---
\newcommand{\CboundA}{0.03342}
\newcommand{\CboundAexact}{0.0334178892}
\newcommand{\CboundB}{0.04775}
\newcommand{\CboundBexact}{0.0477460014}
\newcommand{\CboundC}{0.07641}
\newcommand{\CboundCexact}{0.0764022259}
\newcommand{\CboundD}{0.10506}
\newcommand{\CboundDexact}{0.10505845}
\newcommand{\Cboundzero}{0.019089777}

% --- one-layer remainder constants C' of levy-bfkl-supplement-v6.tex, which is
%     not in this archive, second layer kept with its sign, supremum over
%     x >= x_0 attained at x_0 = 2.35, not printed in this paper ---
\newcommand{\CprimeA}{0.2239}
\newcommand{\CprimeAexact}{0.223862904}
\newcommand{\CprimetriA}{0.2498}
\newcommand{\lnCprimeA}{3.579}
\newcommand{\xplusA}{8.37994}
\newcommand{\XthreshA}{8.37994}
\newcommand{\CprimeB}{0.2476}
\newcommand{\CprimeBexact}{0.24755862}
\newcommand{\CprimetriB}{0.2994}
\newcommand{\lnCprimeB}{2.987}
\newcommand{\xplusB}{5.00325}
\newcommand{\XthreshB}{5.00325}
\newcommand{\CprimeC}{0.2950}
\newcommand{\CprimeCexact}{0.294950052}
\newcommand{\CprimetriC}{0.3985}
\newcommand{\lnCprimeC}{2.469}
\newcommand{\xplusC}{2.79402}
\newcommand{\XthreshC}{2.79402}
\newcommand{\CprimeD}{0.3424}
\newcommand{\CprimeDexact}{0.342341484}
\newcommand{\CprimetriD}{0.4977}
\newcommand{\lnCprimeD}{2.212}
\newcommand{\xplusD}{1.90562}
\newcommand{\XthreshD}{2.35}
\newcommand{\lnCprimemax}{3.58}
\newcommand{\PthreesignA}{9.43794}
\newcommand{\PthreesignB}{7.01960}
\newcommand{\PthreesignC}{5.42281}
\newcommand{\PthreesignD}{4.77429}

% --- the contour constant M on Re gamma = -3/2, and the tail law ---
\newcommand{\fourbbar}{2.77778}
\newcommand{\fourbbarfrac}{\tfrac{25}{9}}
\newcommand{\tailconst}{0.1621}
\newcommand{\Mvalue}{177.5653}
\newcommand{\Mbound}{177.6}
\newcommand{\Munc}{6\times10^{-4}}
\newcommand{\Motwopi}{28.2604}
\newcommand{\Motwopiup}{28.3}
\newcommand{\McollA}{150.5}
\newcommand{\McollB}{152.7}
\newcommand{\MzV}{152.1}
\newcommand{\McollAexact}{150.469}
\newcommand{\McollBexact}{152.667}
\newcommand{\MzVexact}{152.147}

% --- the U(0) = 0 baseline values, not printed in this paper ---
\newcommand{\VUzero}{-1.28858025}
\newcommand{\VUzerofrac}{-\tfrac{835}{648}}
\newcommand{\WUzero}{1.22107}
\newcommand{\rootUzeroA}{16.469}
\newcommand{\rootUzeroB}{8.708}
\newcommand{\rootUzeroC}{4.828}
\newcommand{\rootUzeroD}{3.534}
\newcommand{\collBisolated}{15.7655}
\newcommand{\collBcompA}{149.4}
\newcommand{\collBcompB}{82.6}
\newcommand{\collBcompC}{49.2}
\newcommand{\collBcompD}{38.0}
\newcommand{\VcollA}{0.544753086}
\newcommand{\WcollA}{3.054399}
\newcommand{\UcollA}{-1.83333333}
\newcommand{\VcollB}{-0.149691358}
\newcommand{\WcollB}{2.359955}
\newcommand{\UcollB}{-1.13888889}
\newcommand{\VzV}{0.0}
\newcommand{\WzV}{2.509646}
\newcommand{\UzV}{-1.28858025}

% --- abar_c and the exponent-level statements ---
\newcommand{\chionepp}{-642.5264}
\newcommand{\chizeropp}{33.6576}
\newcommand{\abarcrit}{0.05238}
\newcommand{\abarcritlong}{0.052383205}
\newcommand{\nusqcoeffA}{0.76564}
\newcommand{\nusqcoeffB}{-15.298}
\newcommand{\nusqcoeffC}{-47.424}
\newcommand{\nusqcoeffD}{-79.55}
\newcommand{\Psiinf}{0}
\newcommand{\PsimostnegB}{-0.41390}
\newcommand{\PsimostnegC}{-2.12525}
\newcommand{\PsimostnegD}{-4.09669}
\newcommand{\PsimostnegatB}{0.27}
\newcommand{\PsimostnegatC}{0.40}
\newcommand{\PsimostnegatD}{0.46}
\newcommand{\collAexpA}{4.736}
\newcommand{\collAexpB}{10.58}
\newcommand{\collAexpC}{15.21}
\newcommand{\collAexpD}{18.22}
\newcommand{\collAexpE}{21.98}
\newcommand{\zVexpA}{2.044}
\newcommand{\zVexpB}{5.175}
\newcommand{\zVexpC}{8.708}
\newcommand{\zVexpD}{11.86}
\newcommand{\zVexpE}{15.81}
\newcommand{\collBexpA}{1.305}
\newcommand{\collBexpB}{3.689}
\newcommand{\collBexpC}{6.922}
\newcommand{\collBexpD}{10.11}
\newcommand{\collBexpE}{14.11}

% --- estimated positivity intervals (the rounded contour estimate Motwopiup,
%     pi_0 in closed form) ---
\newcommand{\posloA}{0.512}
\newcommand{\poshiA}{6.642}
\newcommand{\posloAexact}{0.51143717}
\newcommand{\poshiAexact}{6.64266564}
\newcommand{\posloB}{0.711}
\newcommand{\poshiB}{4.164}
\newcommand{\posloBexact}{0.71006916}
\newcommand{\poshiBexact}{4.16402322}
\newcommand{\posloC}{0.973}
\newcommand{\poshiC}{2.568}
\newcommand{\posloCexact}{0.97228692}
\newcommand{\poshiCexact}{2.56833712}
\newcommand{\posloD}{1.237}
\newcommand{\poshiD}{1.861}
\newcommand{\posloDexact}{1.2368374}
\newcommand{\poshiDexact}{1.86140948}

% --- monotone scan of pi_[1](x)/pi_0(x) on [0.2,8], step 0.2 ---
\newcommand{\scanfirst}{2.80633}
\newcommand{\scanlast}{-26.7281}
\newcommand{\scanmindec}{0.5649}
\newcommand{\scanmindecat}{1.6}
\newcommand{\scanmaxdec}{1.14023}

% --- improved kernels: |layer 2|/|layer 1| of the composite
%     abar X0(0,gamma) + abar^2 X1(0,gamma) at abar = 0.05 ---
\newcommand{\ratiocollAA}{0.330}
\newcommand{\ratiocollAB}{0.113}
\newcommand{\ratiocollAC}{0.0386}
\newcommand{\ratiocollAD}{0.00447}
\newcommand{\ratiocollBA}{0.356}
\newcommand{\ratiocollBB}{0.126}
\newcommand{\ratiocollBC}{0.0443}
\newcommand{\ratiocollBD}{0.00544}
\newcommand{\ratiozVA}{0.350}
\newcommand{\ratiozVB}{0.123}
\newcommand{\ratiozVC}{0.0429}
\newcommand{\ratiozVD}{0.00520}
\newcommand{\ratioxonelo}{0.33}
\newcommand{\ratioxonehi}{0.36}

% --- the small-x normalisation at x = 0.5 ---
\newcommand{\pizerohalf}{1.97932}
\newcommand{\pionehalf}{2.4667}
\newcommand{\pionehalfexp}{3.16731}
\newcommand{\smallxA}{2.700}
\newcommand{\smallxB}{2.858}
\newcommand{\smallxC}{3.175}
\newcommand{\smallxD}{3.492}

% --- Mohle rescaling check ---
\newcommand{\mohlecheck}{0.507803462763}
\newcommand{\mohlescaled}{0.761705194144}


==> macros-v3.tex <==
% macros-v3.tex : printed numbers.
% A stored artifact: the program that wrote it is not in this archive.
% Do not hand-edit the numbers.  The comments are maintained by hand.
% The numbers of macros-v2.tex are not repeated here.

% --- the contour constant M the macro names below call proved, from an earlier
%     version of this work, not used in this paper ---
\newcommand{\Mproved}{216}
\newcommand{\Mprovedexact}{215.3795}
\newcommand{\Mpairhalf}{193.4002}
\newcommand{\Mpairthreehalf}{5.98692}
\newcommand{\Mtailproved}{15.9923}
\newcommand{\Mtailleft}{8.53119}
\newcommand{\Mtailmirror}{5.89031}
\newcommand{\Mtailfar}{1.57037}
\newcommand{\Mtailremainder}{0.00042}
\newcommand{\Msqrtroute}{193.475}
\newcommand{\Mmaxminroute}{202.703}
\newcommand{\Mprovedotwopi}{34.4}
\newcommand{\Mprovedotwopiexact}{34.3775}
\newcommand{\CboundprovedA}{0.03651}
\newcommand{\CprimeprovedA}{0.2270}
\newcommand{\lnCprimeprovedA}{3.593}
\newcommand{\CboundprovedB}{0.05393}
\newcommand{\CprimeprovedB}{0.2538}
\newcommand{\lnCprimeprovedB}{3.011}
\newcommand{\CboundprovedC}{0.08876}
\newcommand{\CprimeprovedC}{0.3074}
\newcommand{\lnCprimeprovedC}{2.510}
\newcommand{\CboundprovedD}{0.12359}
\newcommand{\CprimeprovedD}{0.3609}
\newcommand{\lnCprimeprovedD}{2.265}
\newcommand{\lnCprimeprovedmax}{3.60}
\newcommand{\pifivefourth}{76.50}
\newcommand{\chippcontourzero}{48.24}
\newcommand{\chippmajratio}{0.9911}

% --- the sub-abar_c if and only if ---
\newcommand{\abarcritdozen}{0.052383204958}
\newcommand{\nuzeroB}{16.3557579125}
\newcommand{\Rquadcoeff}{0.2519}
\newcommand{\Rminscan}{0.0524839}
\newcommand{\nufourcoeff}{80.919}
\newcommand{\nusqcoeffatabarc}{0}
\newcommand{\chizeroppppahalf}{1542.94849965}
\newcommand{\chioneppppahalf}{-66529.0022588}
\newcommand{\Rvicinitya}{2.51877\times10^{-13}}
\newcommand{\Rvicinityb}{2.51877\times10^{-9}}
\newcommand{\Rvicinityc}{2.51877\times10^{-7}}
\newcommand{\Bathundred}{23.95}
\newcommand{\Batthousand}{67.54}
\newcommand{\Battenthousand}{125.85}
\newcommand{\lnsqhundred}{29.46}
\newcommand{\lnsqthousand}{66.27}
\newcommand{\lnsqtenthousand}{117.82}
\newcommand{\ApBattwenty}{10.03}
\newcommand{\ApBattenthousand}{28.64}
\newcommand{\alphascrit}{0.054855564}
\newcommand{\alphascritround}{0.0549}
\newcommand{\scaletwoloop}{4\times10^{5}}
\newcommand{\scaletwoloopfull}{4.4\times10^{5}}

% --- the all-poles Bessel kernel test ---
\newcommand{\jonezero}{3.83170597}
\newcommand{\bessconst}{2.7094253}
\newcommand{\bessfactor}{1.3547}
\newcommand{\bessrootA}{12.117}
\newcommand{\besskpkA}{427.7}
\newcommand{\bessratioA}{1.824}
\newcommand{\bessrootB}{8.568}
\newcommand{\besskpkB}{72.53}
\newcommand{\bessratioB}{2.057}
\newcommand{\bessrootC}{6.0585}
\newcommand{\besskpkC}{20.68}
\newcommand{\bessratioC}{2.333}
\newcommand{\bessrootD}{4.9467}
\newcommand{\besskpkD}{11.86}
\newcommand{\bessratioD}{2.449}

% --- second-moment framing above abar_c ---
\newcommand{\kpkA}{27.6973}
\newcommand{\rmsYA}{26.22}
\newcommand{\firstmomfracA}{12.651}
\newcommand{\kpkUzeroA}{3767.9}
\newcommand{\lnkpkUzeroA}{8.234}
\newcommand{\collBhalfA}{74.69}
\newcommand{\kpkB}{8.02312}
\newcommand{\rmsYB}{5.1532}
\newcommand{\firstmomfracB}{31.268}
\newcommand{\kpkUzeroB}{77.792}
\newcommand{\lnkpkUzeroB}{4.354}
\newcommand{\collBhalfB}{41.28}
\newcommand{\kpkC}{3.66296}
\newcommand{\rmsYC}{1.0016}
\newcommand{\firstmomfracC}{51.794}
\newcommand{\kpkUzeroC}{11.178}
\newcommand{\lnkpkUzeroC}{2.414}
\newcommand{\collBhalfC}{24.58}
\newcommand{\kpkD}{2.74489}
\newcommand{\rmsYD}{0.4039}
\newcommand{\firstmomfracD}{61.241}
\newcommand{\kpkUzeroD}{5.8545}
\newcommand{\lnkpkUzeroD}{1.767}
\newcommand{\collBhalfD}{19.02}
\newcommand{\collBVnfzero}{-0.458333}
\newcommand{\collBVnfone}{-0.381173}
\newcommand{\collBVnftwo}{-0.304012}
\newcommand{\collBVnfthree}{-0.226852}
\newcommand{\collBVnffour}{-0.149691}
\newcommand{\collBVnffive}{-0.0725309}
\newcommand{\collBVnfsix}{0.00462963}

% --- continuous exponent minima ---
\newcommand{\PsimincontatB}{0.2694166}
\newcommand{\PsimincontB}{-0.4139091}
\newcommand{\PsimincontatC}{0.3972220}
\newcommand{\PsimincontC}{-2.1253796}
\newcommand{\PsimincontatD}{0.4550506}
\newcommand{\PsimincontD}{-4.0971526}

% --- Ao, De la Torre and Gonzalez kernel limit ---
\newcommand{\AoDTGsuba}{2.996954835075}
\newcommand{\AoDTGsubb}{2.973510265268}
\newcommand{\AoDTGsubc}{4.719295674165}
\newcommand{\AoDTGleft}{2.540725690923}
\newcommand{\AoDTGspinsub}{0.200921543028}

% --- Marchesini-Onofri CLT and azimuthal relaxation ---
\newcommand{\Dvalue}{33.657593}
\newcommand{\intabsdeltapizero}{9.869604}
\newcommand{\intabsphimarg}{5.356772}
\newcommand{\kappaonevalue}{2.772589}
\newcommand{\kappatwovalue}{4}
\newcommand{\kappathreevalue}{4.772589}

% --- RGI Green function, Section 4 ---
\newcommand{\rgiDeltanu}{0.25}
\newcommand{\bochcollAa}{-0.00265593}
\newcommand{\bochcollAb}{-0.0851594}
\newcommand{\bochcollAc}{-0.519895}
\newcommand{\bochcollAd}{-0.554882}
\newcommand{\bochcollBa}{-0.00128987}
\newcommand{\bochcollBb}{-0.0432302}
\newcommand{\bochcollBc}{-0.266545}
\newcommand{\bochcollBd}{-0.331953}
\newcommand{\bochzVa}{-0.00160849}
\newcommand{\bochzVb}{-0.0527008}
\newcommand{\bochzVc}{-0.320726}
\newcommand{\bochzVd}{-0.379638}
\newcommand{\semicollAa}{-0.15017}
\newcommand{\semicollAb}{-0.486833}
\newcommand{\semicollAc}{-0.921618}
\newcommand{\semicollAd}{-0.629452}
\newcommand{\semicollBa}{-0.10446}
\newcommand{\semicollBb}{-0.303975}
\newcommand{\semicollBc}{-0.60984}
\newcommand{\semicollBd}{-0.415119}
\newcommand{\semizVa}{-0.113771}
\newcommand{\semizVb}{-0.340361}
\newcommand{\semizVc}{-0.6694}
\newcommand{\semizVd}{-0.453461}
\newcommand{\maxPfivecollAa}{1.0}
\newcommand{\maxPwidecollAa}{1.0}
\newcommand{\maxPfivecollAb}{1.05399}
\newcommand{\maxPwidecollAb}{1.05399}
\newcommand{\maxPfivecollAc}{1.39193}
\newcommand{\maxPwidecollAc}{1.5433}
\newcommand{\maxPfivecollAd}{1.43319}
\newcommand{\maxPwidecollAd}{2.11921}
\newcommand{\maxPfivecollBa}{1.0}
\newcommand{\maxPwidecollBa}{1.0}
\newcommand{\maxPfivecollBb}{1.00159}
\newcommand{\maxPwidecollBb}{1.00159}
\newcommand{\maxPfivecollBc}{1.19577}
\newcommand{\maxPwidecollBc}{1.22504}
\newcommand{\maxPfivecollBd}{1.25693}
\newcommand{\maxPwidecollBd}{1.53461}
\newcommand{\maxPfivezVa}{1.0}
\newcommand{\maxPwidezVa}{1.0}
\newcommand{\maxPfivezVb}{1.00594}
\newcommand{\maxPwidezVb}{1.00594}
\newcommand{\maxPfivezVc}{1.2376}
\newcommand{\maxPwidezVc}{1.28218}
\newcommand{\maxPfivezVd}{1.29455}
\newcommand{\maxPwidezVd}{1.64364}


==> macros-v3b.tex <==
% macros-v3b.tex : the rapidity scan, the minimum eigenvalues of the
% five-point Bochner matrix, the witness row, the scheme spread and the
% inversion-protocol constants, generated by repro/make_macros_v3b.py from
% the files beside it.  The document prints the four rapidities and the three
% short-time eigenvalue rows, all in Section 4, and none of the rest.
% Do not hand-edit.

% --- rapidity of each column of the t = 0.25 tables, Y = t/abar ---
\newcommand{\rgiYa}{5}
\newcommand{\rgiYb}{2.5}
\newcommand{\rgiYc}{1.25}
\newcommand{\rgiYd}{0.833}

% --- minimum eigenvalue of the 5x5 Bochner matrix, scheme/coupling/time ---
\newcommand{\rgimeAaA}{-0.00265593}
\newcommand{\rgimeAaB}{0.0152106}
\newcommand{\rgimeAaC}{0.0985588}
\newcommand{\rgimeAaD}{0.3434}
\newcommand{\rgimeAaE}{0.72463}
\newcommand{\rgimeAbA}{-0.0851594}
\newcommand{\rgimeAbB}{-0.00548783}
\newcommand{\rgimeAbC}{0.0178898}
\newcommand{\rgimeAbD}{0.144655}
\newcommand{\rgimeAbE}{0.483793}
\newcommand{\rgimeAcA}{-0.519895}
\newcommand{\rgimeAcB}{-0.122416}
\newcommand{\rgimeAcC}{-0.0117983}
\newcommand{\rgimeAcD}{0.0159127}
\newcommand{\rgimeAcE}{0.168628}
\newcommand{\rgimeAdA}{-0.554882}
\newcommand{\rgimeAdB}{-0.590445}
\newcommand{\rgimeAdC}{-0.111237}
\newcommand{\rgimeAdD}{-0.000551703}
\newcommand{\rgimeAdE}{0.0478708}
\newcommand{\rgimeBaA}{-0.00128987}
\newcommand{\rgimeBaB}{0.0176728}
\newcommand{\rgimeBaC}{0.101789}
\newcommand{\rgimeBaD}{0.345154}
\newcommand{\rgimeBaE}{0.723289}
\newcommand{\rgimeBbA}{-0.0432302}
\newcommand{\rgimeBbB}{-0.00245914}
\newcommand{\rgimeBbC}{0.0182752}
\newcommand{\rgimeBbD}{0.142053}
\newcommand{\rgimeBbE}{0.474641}
\newcommand{\rgimeBcA}{-0.266545}
\newcommand{\rgimeBcB}{-0.0801707}
\newcommand{\rgimeBcC}{-0.0115907}
\newcommand{\rgimeBcD}{0.00833149}
\newcommand{\rgimeBcE}{0.14289}
\newcommand{\rgimeBdA}{-0.331953}
\newcommand{\rgimeBdB}{-0.255936}
\newcommand{\rgimeBdC}{-0.0808896}
\newcommand{\rgimeBdD}{-0.0062044}
\newcommand{\rgimeBdE}{0.02074}
\newcommand{\rgimeZaA}{-0.00160849}
\newcommand{\rgimeZaB}{0.0171025}
\newcommand{\rgimeZaC}{0.101169}
\newcommand{\rgimeZaD}{0.345074}
\newcommand{\rgimeZaE}{0.723928}
\newcommand{\rgimeZbA}{-0.0527008}
\newcommand{\rgimeZbB}{-0.00267087}
\newcommand{\rgimeZbC}{0.018249}
\newcommand{\rgimeZbD}{0.143201}
\newcommand{\rgimeZbE}{0.477835}
\newcommand{\rgimeZcA}{-0.320726}
\newcommand{\rgimeZcB}{-0.0906208}
\newcommand{\rgimeZcC}{-0.0118703}
\newcommand{\rgimeZcD}{0.0105507}
\newcommand{\rgimeZcE}{0.150859}
\newcommand{\rgimeZdA}{-0.379638}
\newcommand{\rgimeZdB}{-0.330437}
\newcommand{\rgimeZdC}{-0.0891777}
\newcommand{\rgimeZdD}{-0.00456653}
\newcommand{\rgimeZdE}{0.0288805}

% --- the same test on the twenty-one frequencies out to nu = 5, which is the
% scope rgi_green_check_results.json declares for positivity conclusions.  The
% five-point matrix is a principal submatrix of this one, so every cell negative
% there is negative here.  Counted per time, then over all sixty cells. ---
\newcommand{\cellswideD}{5}
\newcommand{\cellswideE}{2}
\newcommand{\cellswidetotal}{26}
\newcommand{\rgiwideBdE}{-0.00625724}
\newcommand{\rgiwideZdE}{-0.000245352}

% --- the Bochner witness row P_t(k dnu), k = 0..4, at abar = 0.05, t = 0.25 ---
\newcommand{\rgiPAzero}{1}
\newcommand{\rgiPAone}{0.968677483}
\newcommand{\rgiPAtwo}{0.88009747}
\newcommand{\rgiPAthree}{0.771089958}
\newcommand{\rgiPAfour}{0.681577708}
\newcommand{\rgiGzeroA}{1.07096}
\newcommand{\rgiPBzero}{1}
\newcommand{\rgiPBone}{0.955083731}
\newcommand{\rgiPBtwo}{0.84272394}
\newcommand{\rgiPBthree}{0.720551405}
\newcommand{\rgiPBfour}{0.627269225}
\newcommand{\rgiGzeroB}{1.19638}
\newcommand{\rgiPZzero}{1}
\newcommand{\rgiPZone}{0.958120793}
\newcommand{\rgiPZtwo}{0.850920037}
\newcommand{\rgiPZthree}{0.73141118}
\newcommand{\rgiPZfour}{0.638815026}
\newcommand{\rgiGzeroZ}{1.16781}

% --- scheme spread in P_t on the validated window, abar = 0.05, t = 0.25 ---
\newcommand{\rgispread}{0.0543}

% --- inversion protocol, from rgi_green_check_results.json ---
\newcommand{\rgilayers}{48{,}000}
\newcommand{\rgilayershi}{96{,}000}
\newcommand{\rgichionehalf}{-18.477594365252703}
\newcommand{\rgichilayermax}{4.926\times10^{-6}}
\newcommand{\rgichilayerone}{1.447\times10^{-9}}
\newcommand{\rgivalidabs}{1.592\times10^{-9}}
\newcommand{\rgivaliddeg}{5.484\times10^{-9}}
\newcommand{\rgifullabs}{1.425\times10^{-3}}
\newcommand{\rgifullrel}{3.599}
\newcommand{\rgifullat}{0.03959545}
\newcommand{\rgidepthdiff}{2.871\times10^{-10}}
\newcommand{\rgichisamplemax}{6.693\times10^{-6}}



==> macros-v3c.tex <==
% macros-v3c.tex : printed numbers.
% A stored artifact: the program that wrote it is not in this archive.

% --- the contour integral M ---
\renewcommand{\Mvalue}{177.5654}

% --- the monotonicity argument on [0.2, 8] ---
\newcommand{\rsecondmax}{32.9}
\newcommand{\scanmindechalf}{0.1412}

% --- second-to-first layer ratio at x -> 0, abar = 0.05 ---
\newcommand{\ratioxzerocollA}{0.9626}
\newcommand{\ratioxzerocollB}{1.0080}
\newcommand{\ratioxzerozV}{0.9980}

% --- roots of the one-, two- and three-layer equations, Table 2 ---
\newcommand{\rootonelayA}{6.639470}
\newcommand{\roottwolayA}{6.642665}
\newcommand{\rootthreelayA}{6.642668}
\newcommand{\rootthreediffA}{5.2\times10^{-9}}
\newcommand{\newtonpredA}{0.00321}
\newcommand{\newtonobsA}{0.00319}
\newcommand{\newtonthirdA}{3.0\times10^{-6}}
\newcommand{\rootonelayB}{4.127038}
\newcommand{\roottwolayB}{4.164224}
\newcommand{\rootthreelayB}{4.164645}
\newcommand{\rootthreediffB}{8.7\times10^{-6}}
\newcommand{\newtonpredB}{0.0391}
\newcommand{\newtonobsB}{0.0372}
\newcommand{\newtonthirdB}{4.2\times10^{-4}}
\newcommand{\rootonelayC}{2.417465}
\newcommand{\roottwolayC}{2.587364}
\newcommand{\rootthreelayC}{2.595691}
\newcommand{\rootthreediffC}{8.5\times10^{-4}}
\newcommand{\newtonpredC}{0.213}
\newcommand{\newtonobsC}{0.170}
\newcommand{\newtonthirdC}{8.3\times10^{-3}}
\newcommand{\rootonelayD}{1.698306}
\newcommand{\roottwolayD}{1.992167}
\newcommand{\rootthreelayD}{2.015173}
\newcommand{\rootthreediffD}{4.3\times10^{-3}}
\newcommand{\newtonpredD}{0.432}
\newcommand{\newtonobsD}{0.294}
\newcommand{\newtonthirdD}{0.023}
\newcommand{\rootthreepct}{0.21}



==> macros-v3d.tex <==
% macros-v3d.tex : grid, witness and inversion-error numbers.
% Generated by repro/make_macros_v3d.py .  Do not hand-edit.

% --- the grid argument for sup C' on [2.35, 42.35] ---
\newcommand{\CprimeLipD}{0.6258}
\newcommand{\CprimeallowD}{0.0313}
\newcommand{\CprimegapD}{0.0451}
\newcommand{\Cprimeratiomin}{1.44}

% --- how far the single leading Regge pole is from the full inversion ---
\newcommand{\leadpoleerrA}{9.7\times10^{-4}}
\newcommand{\leadpoleerrD}{46}

% --- the checkable Bochner witness vector, collB, abar=0.05, t=0.25 ---
\newcommand{\rgiwitBzero}{-0.160463}
\newcommand{\rgiwitBone}{0.495854}
\newcommand{\rgiwitBtwo}{-0.675841}
\newcommand{\rgiwitBthree}{0.495854}
\newcommand{\rgiwitBfour}{-0.160463}
\newcommand{\rgiwitBform}{-0.00128987}
\newcommand{\rgieigbound}{2.4\times10^{-6}}
\newcommand{\rgieigboundwide}{1.0\times10^{-5}}
\newcommand{\semidefBa}{-0.10446}
\newcommand{\semidefAc}{-0.921618}
\newcommand{\maxPwideAd}{2.11921}
\newcommand{\maxPwideAdnu}{2.25}
\newcommand{\widecells}{12}
\newcommand{\wideoverone}{9}

% --- leading Regge pole in the rescaled variable lambda = omega/abar ---
\newcommand{\rgipolezeroB}{2.14592}
\newcommand{\rgipoleoneB}{-0.955919}

% --- declared-grid diagnostics: G_t(0) and max|P_t| over nu <= 5 ---
\newcommand{\rgiGzeromin}{0.2626}
\newcommand{\rgiGzeromax}{3735.2}
\newcommand{\maxPgridA}{2.11921}
\newcommand{\maxPgridB}{1.45183}
\newcommand{\maxPgridC}{1.00628}
\newcommand{\maxPgridD}{1.0}
\newcommand{\maxPgridE}{1.0}

% --- unnormalized total-composition defect at t = s = 0.25 ---
\newcommand{\rgitotalAa}{0.5937}
\newcommand{\rgitotalmin}{0.4279}
\newcommand{\rgitotalmax}{3.579}

% --- quadrature, positivity-gap and monotonicity numbers ---
\newcommand{\Mquadval}{88.54418}
\newcommand{\Mquadspread}{7.2\times10^{-6}}
\newcommand{\posgapA}{2.2\times10^{-6}}
\newcommand{\posgapB}{6.3\times10^{-4}}
\newcommand{\posgapC}{0.0282}
\newcommand{\posgapD}{0.158}
\newcommand{\monodriftA}{2.8245}
\newcommand{\monocurvA}{6.58}
\newcommand{\monodriftB}{2.824}
\newcommand{\monocurvB}{1.645}

% --- four-stage ablation of the t = 0.25 Bochner eigenvalue, abar = 0.05 ---
\newcommand{\ablstageone}{0.065827}
\newcommand{\ablstagetwo}{0.0033249}
\newcommand{\ablstagethreeA}{-0.0047405}
\newcommand{\ablstagethreeB}{-0.00103975}
\newcommand{\ablstagethreeZ}{-0.00148259}


==> macros-v5.tex <==
% macros-v5.tex
% A stored artifact: the program that wrote it is not in this archive.
% Do not edit by hand.

\newcommand{\threshTwo}{0.0523832}
\newcommand{\asymTwo}{0.08333}
\newcommand{\threshFour}{0.0231921}
\newcommand{\asymFour}{0.03333}
\newcommand{\threshSix}{0.0134353}
\newcommand{\asymSix}{0.01786}
\newcommand{\threshEight}{0.00880182}
\newcommand{\asymEight}{0.01111}
\newcommand{\threshTen}{0.00622000}
\newcommand{\asymTen}{0.007576}
\newcommand{\threshTwelve}{0.00463120}
\newcommand{\asymTwelve}{0.005495}
\newcommand{\threshFourteen}{0.00358319}
\newcommand{\asymFourteen}{0.004167}
\newcommand{\threshSixteen}{0.00285522}
\newcommand{\asymSixteen}{0.003268}
\newcommand{\momControlRelErr}{4\times10^{-29}}
\newcommand{\momOddResidual}{9.26\times10^{-33}}
\newcommand{\towerLO}{49.99999792}
\newcommand{\towerRestored}{49.99999729}
\newcommand{\towerFirstLayer}{0.049975}
\newcommand{\towerSmallX}{0.001}
\newcommand{\cmEdgeWidthA}{0.15811388}
\newcommand{\cmEdgeWidthD}{0.38729833}
\newcommand{\realGammaApprox}{-1245.00}
\newcommand{\realGammaEpsilon}{0.01}
\newcommand{\realGammaAtHalf}{0.0924355}
\newcommand{\witnessSpacing}{0.125}
\newcommand{\witnessThreeA}{0.0109945}
\newcommand{\witnessThreeLO}{-0.0141998}
\newcommand{\quarticAtA}{3.71563}
\newcommand{\quarticLOatA}{-3.21448}
\newcommand{\filterPeakPosition}{12.5664}
\newcommand{\filterAtOrigin}{2.6\times10^{-5}}
\newcommand{\filterAtPeak}{3.95}
\newcommand{\filterSuppression}{1.5\times10^{5}}
\newcommand{\filterCoupling}{0.05}
\newcommand{\resolvedEpsilon}{0.1}
\newcommand{\poissonMeanTen}{3.68909}
\newcommand{\poissonEntropyTen}{2.04345}
\newcommand{\geometricEntropyTen}{2.43010}
\newcommand{\poissonEntropyThirty}{2.61301}
\newcommand{\geometricEntropyThirty}{3.44787}
\newcommand{\resolvedTwoSided}{7.37818}
\newcommand{\entropyRapidityA}{10}
\newcommand{\entropyRapidityB}{30}
\newcommand{\alphasSubcritical}{0.055}
\newcommand{\scaleOneLoop}{5.2\times10^{5}}
\newcommand{\chioneathalf}{-18.47759437}
\newcommand{\abarintercept}{0.15005}
\newcommand{\kpkAround}{27.7}
\newcommand{\kpkBround}{8.02}
\newcommand{\kpkCround}{3.66}
\newcommand{\kpkDround}{2.74}
\newcommand{\omegaFOC}{-0.1846}
\newcommand{\alphasAtC}{0.209}
\newcommand{\scaleAtC}{4.4}
\newcommand{\omegaFOD}{-0.8312}
\newcommand{\alphasAtD}{0.314}
\newcommand{\scaleAtD}{1.2}
\newcommand{\rootAsymSmall}{25.794415}
\newcommand{\rootAsymForm}{25.707111}
\newcommand{\rootAsymCoupling}{0.005}
\newcommand{\halfchioneppNFzero}{322.19}
\newcommand{\halfchioneppNFthree}{321.49}
\newcommand{\halfchioneppGap}{0.69}
\newcommand{\phiCheckTerms}{2\times10^{5}}
\newcommand{\phiCheckDiff}{3.2\times10^{-10}}
\newcommand{\phiWorkingDigits}{40}
\newcommand{\satIdentityA}{0.0361518}
\renewcommand{\leadpoleerrA}{1.8\times10^{-3}}
\renewcommand{\leadpoleerrD}{63}
\newcommand{\leadpoleerrAsite}{collB}
\newcommand{\leadpoleerrDsite}{collA}
\renewcommand{\CprimeAexact}{0.223862903}
\renewcommand{\Mtailleft}{8.5311913}
\renewcommand{\Mtailmirror}{5.8903110}
\renewcommand{\rootthreepct}{0.214}
\renewcommand{\rgichilayermax}{4.927\times10^{-6}}
\renewcommand{\rgichisamplemax}{6.694\times10^{-6}}
\renewcommand{\rgivaliddeg}{5.485\times10^{-9}}
\newcommand{\rgichilayerbase}{5.474\times10^{-9}}
\newcommand{\rgilayershihi}{192{,}000}


==> macros-v6.tex <==
% macros-v6.tex
% A stored artifact: the program that wrote it is not in this archive.
% Do not edit by hand.

\newcommand{\chizeroSix}{184406.915848}
\newcommand{\chioneSix}{-13725529.7117}
\newcommand{\chizeroEight}{41289799.9235}
\newcommand{\chioneEight}{-4691052665.59}
\newcommand{\chizeroTen}{14863649017.7}
\newcommand{\chioneTen}{-2.38965549783\times10^{12}}
\newcommand{\chizeroTwelve}{7.84796714336\times10^{12}}
\newcommand{\chioneTwelve}{-1.69458667016\times10^{15}}
\newcommand{\chizeroFourteen}{5.71331689044\times10^{15}}
\newcommand{\chioneFourteen}{-1.59447966492\times10^{18}}
\newcommand{\chizeroSixteen}{5.48478387488\times10^{18}}
\newcommand{\chioneSixteen}{-1.9209665397\times10^{21}}
\newcommand{\threshmodelTwo}{0.0521846458}
\newcommand{\threshmodelFour}{0.0231939829}
\newcommand{\threshmodelSix}{0.0134356422}
\newcommand{\threshmodelEight}{0.00880184999}
\newcommand{\threshmodelTen}{0.00621999928}
\newcommand{\threshmodelTwelve}{0.00463119868}
\newcommand{\threshmodelFourteen}{0.00358318582}
\newcommand{\threshmodelSixteen}{0.00285522093}
\newcommand{\threshmodelrelTwo}{0.00379}
\newcommand{\threshmodelrelSixteen}{7.04\times10^{-10}}
\newcommand{\threshmodelgain}{13.94}
\newcommand{\ctrlthreshTwo}{0.0872552604}
\newcommand{\ctrlthreshFour}{0.0334683435}
\newcommand{\ctrlthreshEight}{0.0111116187}
\newcommand{\ctrlthreshSixteen}{0.00326797388}
\newcommand{\cauchyradius}{0.80}
\newcommand{\cauchypoints}{240}
\newcommand{\cauchymaxG}{2.28777}
\newcommand{\cauchyboundOne}{206.391}
\newcommand{\cauchymarginOne}{90.2}
\newcommand{\cauchyboundEight}{2.58428\times10^{6}}
\newcommand{\cauchymarginEight}{1.13\times10^{6}}
\newcommand{\thresholdTwoAtSpacing}{0.0281805414}
\newcommand{\thresholdTwoLimit}{0.0231921184453}
\newcommand{\thresholdRatio}{2.2587}
\newcommand{\saturationOrder}{2}
\newcommand{\saturationRatio}{2.156}
\newcommand{\resolvedEpsilonB}{0.01}
\newcommand{\resolvedTwoSidedB}{11.9829}
\newcommand{\poissonMeanTenB}{5.99147}
\newcommand{\rgisignlow}{5.0}
\newcommand{\rgisignhigh}{13.3}
\newcommand{\rootroundA}{6.643}
\newcommand{\rootroundB}{4.165}
\newcommand{\rootroundC}{2.597}
\newcommand{\rootroundD}{2.019}
\newcommand{\rgiDeltanuFine}{0.1}


==> macros-v6ptr.tex <==
% macros-v6ptr.tex
% A stored artifact: the program that wrote it is not in this archive.
% Do not edit by hand.

\newcommand{\SMlastsec}{S10}


==> macros-v7.tex <==
% generated by repro/gen_v7.py; do not edit
% fraction of int x |pi_eff| dx on the intervals where pi_eff < 0,
% for the all-poles density in its unmatched form
\newcommand{\lobevarhi}{0.0321}
\newcommand{\lobevarlo}{0.00123}
% declared inputs of the finite-rapidity Bochner scan
\newcommand{\scanabarA}{0.05}
\newcommand{\scanabarB}{0.10}
\newcommand{\scanabarC}{0.20}
\newcommand{\scanabarD}{0.30}
\newcommand{\scantA}{0.25}
\newcommand{\scantB}{0.50}
\newcommand{\scantC}{1.00}
\newcommand{\scantD}{2.00}
\newcommand{\scantE}{4.00}
\renewcommand{\rgiDeltanu}{0.25}


==> macros-v8.tex <==
% generated by repro/gen_v8.py; do not edit
\renewcommand{\lobevarhi}{0.0321}
\newcommand{\lobematchhi}{0.00339}
\newcommand{\zeromatchhi}{5.2948}
\newcommand{\ratiomatchhi}{14.12}
\newcommand{\lobeaphi}{0.000631}
\newcommand{\zeroaphi}{6.04232}
\renewcommand{\lobevarlo}{0.00123}
\newcommand{\lobematchlo}{0.000514}
\newcommand{\zeromatchlo}{12.2474}
\newcommand{\lobeaplo}{0.000483}
\newcommand{\zeroaplo}{12.2475}
\newcommand{\stripfailratio}{-0.371}
\newcommand{\stripfaileps}{0.403}
\renewcommand{\chizeropp}{33.6576}
\renewcommand{\chionepp}{-642.5264}
\renewcommand{\abarcrit}{0.05238}
\renewcommand{\bessconst}{2.7094253}


==> macros-v9.tex <==
% generated by repro/gen_v9.py; do not edit
\newcommand{\cauchyrad}{0.25}
\newcommand{\throne}{0.052383}
\newcommand{\thrtwo}{0.023192}
\newcommand{\thrthree}{0.013435}
\newcommand{\convfaileps}{0.4594}
\newcommand{\convfailratio}{-0.3395}
\newcommand{\shiftpi}{52.15}
\newcommand{\shiftphi}{-23.73}
\newcommand{\shiftb}{-2.92}
\newcommand{\archiveprinted}{123}
\newcommand{\archiveregen}{123}
\newcommand{\archiveretired}{0}
\newcommand{\cellsA}{12}
\newcommand{\cellsB}{9}
\newcommand{\cellsC}{6}
\newcommand{\cellsD}{3}
\newcommand{\cellsE}{0}
\newcommand{\cellstotal}{30}
\newcommand{\weightsixteen}{3.92}
\newcommand{\weightlimit}{4.35}
\newcommand{\ratiohi}{11.86}
\newcommand{\damphi}{0.0843}
\newcommand{\ratiolo}{427.7}
\newcommand{\damplo}{0.00234}
\newcommand{\bbarvalue}{0.69444444}
\newcommand{\dthirteenval}{-\tfrac12}
\newcommand{\alphasScanA}{0.0524}
\newcommand{\alphasScanB}{0.105}
\newcommand{\alphasScanC}{0.209}
\newcommand{\alphasScanD}{0.314}
\newcommand{\rootcountpoints}{60}
\newcommand{\rootcountreach}{20000}
\newcommand{\rootcountreachsmall}{400}
\newcommand{\rootcountmargin}{0.01}
\newcommand{\rootcountfar}{0.006}
\newcommand{\inversionabscissalo}{6.91}
\newcommand{\inversionabscissahi}{110.5}
\newcommand{\rootcountedge}{-3}
\newcommand{\rootcountwidepoints}{252}
\newcommand{\rootcountwidefreq}{21}
\newcommand{\thrsuppconst}{\tfrac15}
\newcommand{\rootcountrzero}{1238.65}
\newcommand{\plusepshiA}{0.1951}
\newcommand{\plusepsloA}{0.4923}
\newcommand{\plusepshiD}{0.0003866}
\newcommand{\plusepsloD}{0.02469}
\newcommand{\plusratiohiD}{-0.3334}
\newcommand{\plusratioloD}{-0.1693}
\newcommand{\plusabarD}{10^{-4}}
\newcommand{\acabarzero}{0.40142}
\newcommand{\acabarfour}{0.40349}
\newcommand{\clayertwoinf}{\tfrac{157}{210}}
\newcommand{\clayeronebound}{\tfrac{12451}{4050}-\tfrac{\pi^2}{12}}

